CroCoDai: A Stablecoin for Cross-Chain Commerce

Decentralized Finance (DeFi), in which digital assets are exchanged without trusted intermediaries, has grown rapidly in value in recent years. The global DeFi ecosystem is fragmented into multiple blockchains, fueling the demand for cross-chain commerce. Existing approaches for cross-chain transactions, e.g., bridges and cross-chain deals, achieve atomicity by locking assets in escrow. However, locking up assets increases the financial risks for the participants, especially due to price fluctuations and the long latency of cross-chain transactions. Stablecoins, which are pegged to a non-volatile asset such as the US dollar, help mitigate the risk associated with price fluctuations. However, existing stablecoin designs are tied to individual blockchain platforms, and trusted parties or complex protocols are needed to exchange stablecoin tokens between blockchains. Our goal is to design a practical stablecoin for cross-chain commerce. Realizing this goal requires addressing two challenges. The first challenge is to support a large and growing number of blockchains efficiently. The second challenge is to be resilient to price fluctuations and blockchain platform failures. We present CroCoDai to address these challenges. We also present three prototype implementations of our stablecoin system, and show that it incurs small execution overhead.

==> sec/complete_experiments_table.tex <==
\Cref{tab:end_to_end_experiments_complete} displays the gas costs of the individual transactions in the four end-to-end processes of \Cref{sec:end_to_end_experiments} -- stablecoin creation and cross-chain transfer for both \name{} and the DSS baseline. For each transaction, we display the contract, function, and chain, combined with the step number of this transaction in the end-to-end process, and the total gas cost. \Cref{tab:end_to_end_experiments} contains the same results, but groups transactions can that occur within the same block together.

\setlength{\tabcolsep}{5pt}
\begin{table}
\centering
\caption{Computation costs (units of gas) of the various steps in \name and the DSS baseline. Computations on the relay chain (i.e., Ethereum in the case of the DSS) are in \textbf{bold}.}
\label{tab:end_to_end_experiments_complete}
\begin{tabular}{r|llll}
 & \multicolumn{2}{c}{\name} & \multicolumn{2}{c}{DSS baseline} \\ 
 contract (function), chain & creation & transfer & creation & transfer \\ \toprule
\texttt{GemCoin} (approve), {A} & 
    1.\ 46815 & 
    1.\ 46693 & 
    1.\ 46815 &  
     \\
\texttt{GemJoin} (join), {A} & 
    2.\ 99306 & 
     & 
     & 
     \\
\texttt{Vat} (frob), {A} & 
    3.\ 162631& 
     & 
     & 
     \\
\texttt{Vat} (hope), {A} & 
    4.\ 44247 & 
    & 
     & 
     \\
\texttt{DaiJoin} (exit), {A} & 
    5.\ 113538 &  
    & 
     & 
    \\
\texttt{CCTransfer} (addOutgoing), {A} & 
    & 
    2.\ 170392 & 
    & 
    \\
\texttt{Relay} (approve), {A} & 
    & 
    3.\ 49352 & 
     &  
     \\
\texttt{GemBridge} (deposit), {A} & 
    & 
     & 
    2.\ 197221 & 
     \\
\texttt{WrDai} (burn), {A} & 
    & 
     & 
     & 
    1.\ 27762 \\
\texttt{CCTransfer} (addTransfer), \textbf{R} & 
    & 
    \dbcb{4.\ 170392} & 
    & 
     \\
\texttt{WrGemCoin} (mint), \textbf{R} & 
    & 
    & 
    \dbcb{3.\ 71498} & 
     \\
\texttt{WrGemCoin} (approve), \textbf{R} & 
    & 
    & 
    \dbcb{4. 46815} & 
     \\
\texttt{GemJoin} (join), \textbf{R} & 
    & 
    & 
    \dbcb{5. 94506} & 
     \\
\texttt{Vat} (frob), \textbf{R} & 
    & 
    & 
    \dbcb{6. 162631} & 
     \\
\texttt{Vat} (hope), \textbf{R} & 
    & 
    & 
    \dbcb{7. 44247} & 
     \\
\texttt{DaiJoin} (exit), \textbf{R} & 
    & 
    & 
    \dbcb{8. 113538} & 
     \\
\texttt{Dai} (approve), \textbf{R} & 
    & 
    & 
    \dbcb{9. 46693} &
    \dbcb{3. 46693} \\
\texttt{DaiBridge} (deposit), \textbf{R} & 
    &  
    & 
    \dbcb{10. 190796} & 
    \dbcb{4. 190796} \\
\texttt{DaiBridge} (withdraw), \textbf{R} & 
    & 
    & 
    & 
    \dbcb{2. 56527} \\
\texttt{WrDai} (mint), {A} & 
    & 
    & 
    11. 71498 & 
     \\
\texttt{CCTransfer} (addIncoming), {B} & 
    & 
    5. 136151& 
    & 
     \\
\texttt{Relay} (approve), {B} & 
    & 
    6. 49352 & 
    & 
     \\
\texttt{WrDai} (mint), {B} & 
    & 
    & 
    & 
    5. 71498 \\ \midrule
Total\ (coin chains) & 466537 & 451940 & 315534 & 99260 \\
\textbf{Total (relay chain)} & \textbf{0} & \textbf{170392} & \textbf{770724} & \textbf{294016} \\
\bottomrule
\end{tabular}
\end{table}

==> sec/distribution_fit.tex <==
The GBM is usually assumed to follow a normal distribution. In previous simulations we used
normal distributions to simulate the returns. As mentioned by many papers, distribution of
stock returns is usually more heavy-tailed and Student’s t-distribution is better fit (see, e.g., \cite{li2020review,kelly2014tail}). When comparing residual sum of squares for normal and t-distribution on
returns of ETH, we get a  residual sum of squares (RSS) that is approximately equal to 31900 and 14000 for the normal and $t$-
distribution, respectively. Moreover, the fitted $t$-distribution has a lower RSS for all other assets as
well.
In \Cref{fig:dist_fit}, we have displayed a comparison of the normal and $t$-distribution fitted on Ethereum and
Solona returns. As such, we prefer to use the $t$-distribution for the risk analysis in this paper.

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/distribution.png}
\caption{Comparison between t-distribution and normal distribution fitted on historical
returns.}\label{fig:dist_fit}
\end{figure*}

==> sec/existing_approaches.tex <==

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.8]{figures/auction_model1.pdf}
\caption{Single contract, centralized exchange.}
\end{figure}

\textbf{Single Chain + Exchange.} 

\begin{enumerate}
\item The auctioneer creates a smart contract on blockchain $j'$ and uses it to escrow the NFT.

\item Each user $i$ uses a cryptocurrency exchange to exchange their $x_{ij}$ $j$-tokens on blockchain $j$ to $x^*_{ij} = x_{ij} p_j / p_{j^*}$ $j'$-tokens on blockchain $j^*$. In particular, they send the tokens from their wallet to the exchange wallet, then exchange, then send it to their wallet on blockchain $j'$. Finally, they send their $j'$-tokens from the wallet on blockchain $j'$ to the smart contract on chain $j'$

\item At time $t^*$, the smart contract executes its logic: the seller receives the winning bid, the winner receives the NFT, and all other bidders receive a refund.
\end{enumerate}

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.8]{figures/auction_model2.pdf}
\caption{Multiple contracts.}
\end{figure}

\textbf{Multiple smart contracts.}
\begin{enumerate}
\item The auctioneer creates a smart contract on each blockchain, and escrows the NFT in the smart contract on chain $j'$.

\item Each user $i$ places a bid $b_{ij} = v_i/p_{jt}$ if $x_{ij} > b_{ij}$, and escrows $b_{ij}$ in the smart contract on blockchain $j$.

\item At time $t^*$, the auctioneer combines the bids on the different contracts to determine the winning bid. The auctioneer makes calls to the smart contracts on all blockchains to specify the contract logic: the seller receives the winning bid, the winner receives the NFT, and all other bidders receive a refund.

\item The bidder validate the execution logic and collectively create a commit vote. If one or more user disagree, the process aborts and all assets are returned. If the commit vote is constructed successfully, it is sent to all contracts and the assets are transferred.
\end{enumerate}

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.8]{figures/auction_model3.pdf}
\caption{Single contract, wrapped tokens and AMMs.}
\end{figure}

\textbf{Single Chain + \xclaim.} 

\begin{enumerate}
\item The auctioneer creates a smart contract on blockchain $j'$ and uses it to escrow the NFT.

\item Each user $i$ sends their $x_{ij}$ tokens to a vault, which then creates $x_{ij}$ wrapped $j$-tokens on chain $j'$. Next, user $i$ swaps her wrapped $j$-tokens for $j'$-tokens using an AMM, and sends the $j'$tokens to the smart contract on chain $j'$

\item At time $t^*$, the smart contract executes its logic: the seller receives the winning bid, the winner receives the NFT, and all other bidders receive a refund.
\end{enumerate}

\subsection*{Evaluation of Existing Approaches}
A summary of our evaluation of the existing approaches is depicted in \Cref{tab:existing_approaches}.


\begin{table}[h]
\centering
\caption{Evaluation of the Different Approaches}
\label{tab:existing_approaches}
\begin{tabular}{r|cccc|c}
 \rot{} & \rot{Centralized Exchange} & \rot{{Cross-Chain Deal}} & \rot{{Wrapped Tokens}} & \rot{{\xclaim}} & \rot{{Our Solution}} \\ \toprule
Safety/Liveness & \badcross & {\goodcheck} & {\badcross} & {\goodcheck} & {\goodcheck}  \\
Dep.\ Efficiency & \goodcheck & {\goodcheck} & {\badcross} & {\badcross} & {\goodcheck}  \\
Local Users & \goodcheck & {\badcross} & {\goodcheck} & {\goodcheck} & {\goodcheck}  \\ \midrule
Fin.\ Safety & \meh & \meh & \meh & \meh & \good\good \\
{Fin.\ Liveness} & \good & \good & \bad & \bad & \good \\
\bottomrule
\end{tabular}
\end{table}


==> sec/list_of_symbols.tex <==
A list of symbols used in this paper can be found in \Cref{tab:list_of_symbols}.


\begin{table}[h]
\caption{List of symbols.}
\label{tab:list_of_symbols}
\centering
\begin{tabular}{cl}
symbol & description \\ \toprule
$p_{m\,t}$ & base price of token $m$ at time $t$ \\
$p_{m\,o\,t}$ & price of token $m$ at time $t$, as reported by oracle $o$ \\
$\mu_{m}$ & mean drift of the stochastic process $p_{m\,t}$ \\
$\sigma^2_{m}$ & variance of the stochastic process $p_{m\,t}$ \\
$\mu_{m\,o}$ & mean of the random variable $p_{m\,o\,t} - p_{m\,t}$ \\
$\sigma^2_{m\,o}$ & variance of the random variable $p_{m\,o\,t} - p_{m\,t}$ \\
$y_j$ & collateral token type of CDP $j$ \\
$c_{j\,t}$ & number of collateral tokens held in CDP $j$ at time $t$\\
$D_{j\,t}$ & debt of CDP $j$ at time $t$\\
$\zeta_{m}$ & debt ceiling of token type $m$ \\
$\zeta'$ & total debt ceiling of the failed/compromised asset types \\
$\gamma$ & liquidation ratio \\
$\lambda$ & maximum contribution of each individual asset type during convex optimization \\
$\theta$ & system failure threshold \\
$\mathcal{J}_t$ & set of all CDPs at time $t$ \\
$M$ & number of tokens \\
$O$ & number of price feeds \\
$U$ & number of users \\
\bottomrule
\end{tabular}
\end{table}

\newpage

==> sec/system_model.tex <==

% In the following, we describe our model for cross-chain token transfers. 

\subsection{Entities}

Our system model has the following types of entities. In the following, we use the notation $[n]$ for $\{1,\ldots,n\}$. A list of symbols can be found in \Cref{tab:list_of_symbols} in \Cref{sec:list_of_symbols}.

\begin{itemize}[leftmargin=12pt]

\item \textbf{Token:} a type of cryptocurrency or an NFT (although typically the former due to the better availability of price information for cryptocurrencies). We denote the number of different tokens in the system by $M \geq 2$.

\item \textbf{Governance Token:} this is a type of cryptocurrency that gives holders the right to vote on decisions that affect the functioning of the crypto-backed stablecoin. The governance token cannot be used as collateral for the stablecoin.

\item \textbf{Blockchain (or \textit{chain}):} an immutable, distributed ledger that tracks the ownership of its tokens. We assume that each chain either supports smart contracts or that a \textit{wrapped} version of its native tokens exist on a chain that does (e.g., WBTC \cite{werner2021sok}). We denote the number of supported chains by $B \geq 2$, and the chain of token $m \in [M]$ by $b_m \in [B]$.

\item \textbf{Consensus Node:} is responsible for maintaining the blockchain, e.g., through the creation and/or validation of new blocks. The nature of the consensus nodes depends on the blockchain's consensus protocol -- examples include variations of proof-of-work, proof-of-stake, or Byzantine Fault Tolerance (BFT) protocols. Each consensus node has some amount of \textit{consensus power} -- e.g., processing power in proof-of-work, staked tokens in proof-of-stake, or a private key in a BFT protocol. 

\item \textbf{User:} owns blockchain tokens and seeks to exchange them for tokens on another chain.  
We denote the number of users in our system by $U \geq 1$.

% \item \textbf{Wallet:} a collection of private keys controlled by a user. For simplicity, we assume that each user $i$ only has a single wallet $w_{i\,b}$ on each chain $b$. If tokens are transferred from a wallet $w_{i\,b}$ to another wallet $w_{i'\,b}$, then this represents a blockchain transaction in which the tokens are sent from an address with a key controlled by user $i$ to an address with a key controlled by user $i'$.

\item \textbf{Smart contract:} a software program on a blockchain that may hold tokens which can be sent to other contracts or wallets depending on the program's internal logic.

%\item \textbf{EX:} controls a set of wallets of different chains -- users may send (receive) tokens to (from) the wallets controlled by the EX based on their interactions with the EX's user interface.
%
%\item \textbf{DEX:} allows for the automated exchange of token types that exist on the same blockchain. We assume that there are $K \geq 1$ exchanges (EXs and DEXs) in total.

\item \textbf{Vault:} a smart contract or address that holds tokens as collateral, and to/from which tokens can be sent/received leading to the possible creation/destruction of stablecoins managed by another smart contract.

\item \textbf{Price Oracle:} a type of user who provides price information to the system \cite{liu2021first}, e.g., Chainlink \cite{breidenbach2021chainlink}. We denote the number of price oracles in our system by $O \geq 1$. Each oracle $o \in [O]$ can provide price information for any selection of tokens. Let $p_{m\,o\,t}$ be the price of token $m \in [M]$ reported by oracle $o \in [O]$ at time $t \geq 0$. A \textit{price feed} is a sequence of prices for a given token $m$ reported by an oracle $o$.

\end{itemize}

\subsection{Token Price Model} 
\label{sec:token_price_model}

%We represent time as a sequence of $T \geq 1$ phases, and 
%%We deliberately choose a representation of time that is too abstract to represent factors that have negligible impact on long time scales, such as differences between block creation processes on different blockchains and network latency. 
%use $x_{i\,j\,m\,t} \geq 0$ to denote the total number of tokens of type \mbox{$m \in [M]$} (on blockchain $b_m$) sent by user $i$ to user $j$ in phase \mbox{$t \in [T]$}.  
%%We denote the number of tokens of type $m \in [M]$ in wallet $i \in [N]$ by $x_{i\,b}$. 
%We denote a \textit{system execution} by $\x = (x_{i\,j\,m\,t})_{i,j \in [N], m \in [M], t \in [T]}$. We note that this is a generalization of the use of matrices in cross-chain deals, as we consider the phase and token type of each transfer in addition to the involved users \cite{herlihy2021cross}. A protocol $\Pi$ specifies a set of \textit{feasible} executions, $\X_{\Pi}$, and an ideal execution $\x_{\Pi} \in \X_{\Pi}$. For each user $i$, let $y_{i\,m\,0}$ be the number of tokens of type $m$ owned before the start of phase $1$, and let
%$$
%y_{i\,m\,t}(\x) = y_{i\,m\,0} + \sum_{t' =1 }^t \sum_{j =1}^N \left(x_{j\,i\,m\,t} - x_{i\,j\,m\,t}\right)
%$$ 
%denote the total number of tokens of type $m$ held by user $i$ at the end of phase $t \in [T]$ given execution $\x$. Let
%$\y(\x) = (y_{i\,m\,T}(\x))_{i \in [N], m \in [M]}$ represent the \textit{outcome} of execution $\x$, i.e., the total number of tokens of type $m$ held by each user $i$ at the end of the final phase. If $\x$ is inconsequential, we write $\y$ instead of $\y(\x)$ for brevity.

%Each user $i \in [N]$ has a \textit{utility} $u_i(\y)$ for each outcome $\y$. If \mbox{$u_i(\y) \geq 0$}, then outcome $\y$ is said to be \textit{acceptable} to user $i$. We also assume that there is a \textit{social welfare function} $W := \mathbb{R}^{N+M} \rightarrow \mathbb{R}$, where $W(\y) > W(\y')$ if outcome $\y$ is more socially desirable than $\y'$. An outcome $\y$ such that $W(\y) = \max_{\y' \in \mathbb{R}^{N+M}} W(\y')$ is called \textit{socially optimal}.

In our model, token prices are represented in terms of their exchange rate with a non-volatile base asset, e.g., the US dollar (the \textit{numéraire}). We denote the base price of token $m \in [M]$ at time $t > 0$ given by $p_{m\,t}$, and the initial base price of token $m$ by $p_{m\,0}$. (Here, $t=0$ represents an arbitrary start point of time.) Given a batch of $k \geq 0$ tokens of type $m$, the \textit{value} of this batch at time $t$ is given by $k p_{m\,t}$. We assume that the price of token $m$ at time $t$ returned by an honest price oracle $o \in [O]$ equals $p_{m\,o\,t} \triangleq p_{m\,t} + \Delta_{m\,o}$, where $\Delta_{m\,o}$ is a random variable with a normal/Gaussian distribution \cite{ross2011elementary} with mean $\mu_{m\,o} \in \mathbb{R}$ and variance $\sigma^2_{m\,o} > 0$. This assumption is motivated by the common assumption that measurement errors have a normal distribution, e.g., in linear regression \cite{dobson2018introduction}.
%In principle, each exchange may have a exchange rates for tokens that may be different from the base price, i.e., each exchange $k \in [K]$ has its own exchange rate $p_{m\,k}(t) / p_{m'\,k}(t)$ for tokens $m,m' \in [M]$ at the end of phase $t$.

To model the evolution of token prices over time, we use \textit{Geometric Brownian Motion} (GBM). This is a common choice in the financial literature on asset prices \cite{ross2011elementary} and related work on stablecoins, e.g., by Salehi et al.\ \cite{salehi2021red}, particularly due to the GBM's role in the Black-Scholes formula for option prices.  A stochastic process $S_t$
that follows GBM is defined using a stochastic differential equation:
\begin{equation}
dS_t = \mu S_t dt + \sigma S_t d W_t,
\label{eq:gmb_definition}
\end{equation}
where $\mu$ determines the drift of $S_t$ (i.e., its expected change per unit of time), $\sigma$ represents the volatility of $S_t$ (i.e., the variance of the change), and
% \textcolor{red}{please explain mu and sigma. Wiki says these are: mu  ('the percentage drift') and 
% sigma  ('the percentage volatility') are constants. I suppose statistically they are also mean and std but these two notions need to be made explicit and reconciled}
$W_t$ is the Wiener process that represents standard Brownian motion \cite{ross2011elementary}. 
% As such, $S_t$ represents a process such that the difference between $\log(S_{t+t'}) - \log(S_{t})$  
% The process \eqref{eq:gmb_definition} has an analytical solution,
% \begin{equation}
% S_t = S_0  \cdot \left\{ \left( \mu - \frac{\sigma^2}{2}\right) + \sigma W_t\right\},
% \label{eq:gbm_analytical_solution}
% \end{equation}
% which can be used to efficiently simulate asset prices (see  \Cref{sec:alternate_simulation_methods} for a detailed discussion).
In this model, each token price process $p_{m\,t}$, $t \geq 0$, can be represented using a process defined as in \Cref{eq:gmb_definition}. Essentially, this means that the logarithm of the relative difference of token prices, $\log\left(p_{m\,t+t'} / p_{m\,t}\right)$, is normally distributed for all $t' > 0$ with mean and variance dependent on $t'$.
% In our case, when modeling prices, $S_t$ denotes the log returns of a given asset. 
Unlike \cite{salehi2021red}, we consider a setting with multiple assets; i.e., we have a stochastic process $S_{m\,t}$ for each token $m$ with its own mean $\mu_m$ and variance $\sigma^2_m$. In this setting, we must also consider
the \textit{covariance} between the token prices \cite{ross2011elementary}, as cryptocurrency prices are often highly correlated -- we will discuss this in more detail in \Cref{sec:analysis}. More details about how the standard GBM can be used to simulate asset prices can be found in \Cref{sec:alternate_simulation_methods}.

The standard GBM as decribed above is based on the normal distribution, i.e., $\log(S_{t+t'}/S_t)$ has a normal distribution. However, it is known from the academic literature that the probability distribution of stock price fluctuations is usually more heavy-tailed and that Student’s $t$-distribution is often a better fit \cite{kelly2014tail,li2020review}.  This is also visible in the data for price changes in our dataset -- see \Cref{fig:dist_fit} in \Cref{sec:distribution_fit}.
% When comparing residual sum of squares for normal and $t$-distribution on returns of Ethereum, we get RSS equal approx. to 31900 and 14000 for normal and $t$-distribution respectively. Moreover fitted t-distribution has lower RSS for all other assets as well. 
As such, we will focus on the $t$-distribution in our analysis. Although the $t$-distribution does not allow for an analytical solution for the asset price change after each individual time slot (e.g., as per \eqref{eq:gbm_analytical_solution} in \Cref{sec:alternate_simulation_methods}), 
% analogous to \Cref{eq:gbm_analytical_solution}, 
we can use Monte Carlo simulation to analyze its behavior, as we discuss in more detail in \Cref{sec:analysis}.

\subsection{DSS Execution Model}

Let $\mathcal{J}_t$ denote the set of all CDPs at time $t$, and $c_{j\,t}$ the total number of collateral tokens held in CDP $j \in \mathcal{J}_t$ at time $t$.
 Let $D_{j\,t}$ be the outstanding debt resulting from Dai withdrawals/deposits from/to CDP $j \in \mathcal{J}_t$. Each CDP is associated with a specific token type -- let $y_j$ be the token type of CDP $j$. Debt is subject to fees, i.e., $D_{j\,t+1} = (D_{j\,t}) ^ {1 + \delta}$, where $\delta$ represents the stability fee. 
 We denote the number of stablecoins held by user $u \in [U]$ at time $t$ by $h_{u\,t}$. 
 We note that, in principle, $\sum_{u \in [U]} h_u \leq \sum_{j \in \mathcal{J}} D_{j\,t}$, as stablecoins are created and transferred to a user account either through withdrawal from a CDP (in which case the created  stablecoins and debt are equal) or from a vault through the Dai savings rate (in which case the created stablecoins cannot exceed the excess debt). However, we will consider attacks in \Cref{sec:threat_model} that can cause this assumption to be violated. 

We formalize the liquidation criterion as follows: for each CDP $j \in \mathcal{J}_t$ and $t \geq 0$, it must hold that 
% \begin{equation}
$
p_{y_j\,t} c_{j\,t}/y_{j\,t} > \gamma,
$
% \label{eq:liquidation_condition}
% \end{equation}
where $\gamma$ is the liquidation ratio -- if this condition does not hold, then CDP $j$ can be liquidated through a collateral auction. We assume that under standard conditions (i.e., the absence of an attack or sudden price collapse), collateral auctions are concluded successfully, i.e., a sufficient amount of stablecoins is raised to close the position. No user can create debt if the result would violate the liquidation criterion. We also note that price fluctuations do not affect the liquidation criterion, nor does the Dai savings rate as the proportional effect on all CDP debts is the same.

We denote the debt ceiling for each token type $m \in [M]$ by a fraction $\zeta_m \in [0,1]$, i.e., the total debt in CDPs of type $m$ relative to the system's total debt cannot exceed $\zeta_m$. (Debt ceilings are specified in absolute terms in DSS contracts, but we assume that the difference is negligible for short periods, e.g., for escrow.)
% (Although debt ceiling are specified in absolute terms in DSS contracts, we represent them as fractions of the total to simplify the analysis in \Cref{sec:analysis}.)
% Let $\mathcal{J}_m = \{j \in \mathcal{J}:y_j = m\}$ be set of all CDPs of type $m$, and $D^*_{m\,t} = \sum_{j \in \mathcal{J}_m} D_{j\,t}$ represent the total debt associated with CDPs of type $m$ at time $t$. 
The debt ceilings are used to enforce
$
% \begin{equation}
\sum_{\substack{j \in \mathcal{J}_t \\ y_j = m}} D_{j\,t} < \zeta_m \sum_{j \in \mathcal{J}_t} D_{j\,t}
% \label{eq:debt_ceiling}
% \end{equation}
$ for all $m \in [M]$.
 Let $D_t^* = \sum_{j \in \mathcal{J}_t} D_{j\,t}$ and $C^*_t = \sum_{j \in \mathcal{J}_t} p_{y_j \, t}c_{j\,t}$ denote the total debt and the total collateral value across the system at time $t$, respectively.

\subsection{Threat Model}
\label{sec:threat_model}

We make the following assumptions about the system entities.
% \paragraph*{Governance Token Holders.}
% \paragraph*{Consensus Nodes.} We assume that a majority 
We assume that a majority of the governance token holders are honest. For each underlying blockchain, we assume that it is either compromised or not. If it is not compromised, we assume that it guarantees safety and liveness for all of its transactions. However, both safety and liveness can be violated in a compromised blockchain -- in particular, transactions in which collateral is sent to/from a CDP can be overturned. 
% In this case, a node is \textit{honest} if it acts in agreement with the protocol as described, and \textit{online} means that it is able to communicate with other nodes.
% For a typical blockchain, this assumption is sufficient to guarantee \textit{liveness} -- i.e., transactions by honest nodes are eventually processed -- and \textit{safety} -- i.e., no pair of conflicting transactions are ever processed. 
% However, we will also consider an attack in which a majority of the consensus power in a single blockchain is compromised. 
For the price oracles, we assume that a majority is online and honest at all times, but that dishonest oracles can report arbitrary prices.

\subsection{System Requirements}
\label{sec:requirements}

The central requirement that we focus on in this paper is the following:
\begin{enumerate}
\item[(*)] \textbf{Full Backing.} At any time $t \geq 0$, the ratio of the value of the collateral tokens to the total number of stablecoins in the system exceeds a safety threshold $\theta$, i.e.,
\begin{equation}
C^*_t / D^*_t > \theta.
\label{eq:full-backing}
\end{equation}
\end{enumerate}
We assume that $\theta>1$, i.e., system failure occurs when the ratio of the collateral value to the debt gets sufficiently close enough to $1$. The motivation behind this requirement is as follows: the fundamental guarantee that underpins crypto-backed stablecoins is that in the event of a system shutdown, there is enough collateral in the vaults to refund each user who holds $h$ stablecoins with a basket of tokens whose value equals $h$ units of the pegged asset. If price fluctuations or an attack would cause this requirement to be violated, then we can reasonably expect the stablecoin to lose its peg. This would be detrimental to the user experience as their tokens held in escrow would depreciate, causing financial losses.

Due to random price fluctuations, we cannot guarantee with absolute certainty that \eqref{eq:full-backing} will hold in all circumstances. However, we use our analysis to show that for reasonable choices of $\theta$ and the liquidation ratio $\gamma$, the probability that \eqref{eq:full-backing} is violated after a medium-length period (i.e., one day) is very small for historical data. We do this both for portfolios that approximate the current state of the DSS (as of late April 2023), and portfolios that are optimized for minimal risk given a selection of possible single-chain or cross-chain tokens. In \Cref{sec:analysis}, we also investigate under which conditions \eqref{eq:full-backing} continues to hold in the event of a black swan event such as a sudden token price collapse or a 51\% attack on a blockchain. 
% \textcolor{red}{can we reinforce this assertion with a statement on our further analysis on identification of weakest links and mitigation of risks (in lines with what we discussed)?}

Furthermore, we require the following properties under the threat and token price model.
\begin{enumerate}[leftmargin=15pt]

\item \textbf{Safety.} Users do not lose tokens during stablecoin transfers.

\item \textbf{Liveness.} Stablecoin transfers eventually happen.

\item \textbf{Safety of Collateral} (informal). The probability that a minority of corrupted oracles cause a CDP that is not underwater to be inadvertently liquidated is small.
\end{enumerate}
More formally, for the last property we consider a minority of corrupted price oracles whose goal is to convince the protocol to accept a price $p^*$ instead of a true base price $p$ -- safety of collateral then holds if their probability of success vanishes exponentially as $|p-p^*|$ increases (see also \Cref{thm:corrupted_price_feeds} in \Cref{sec:technical_safety}).

As we will see in \Cref{sec:analysis}, the former two properties largely follow from results in the existing scientific literature. The latter is a result that we prove for the multi-chain setting in \Cref{sec:analysis}, but which is also applicable in the single-chain setting.


